A new heuristic algorithm for fast k-segmentation

The $k$-segmentation of a video stream is used to partition it into $k$ piecewise-linear segments, so that each linear segment has a meaningful interpretation. Such segmentation may be used to summarize large videos using a small set of images, to identify anomalies within segments and change points between segments, and to select critical subsets for training machine learning models. Exact and approximate segmentation methods for $k$-segmentation exist in the literature. Each of these algorithms occupies a different spot in the trade-off between computational complexity and accuracy. A novel heuristic algorithm is proposed in this paper to improve upon existing methods. It is empirically found to provide accuracies competitive with exact methods at a fraction of the computational expense. The new algorithm is inspired by Lloyd's algorithm for K-Means and Lloyd-Max algorithm for scalar quantization, and is called the LM algorithm for convenience. It works by iteratively minimizing a cost function from any given initialisation; the commonly used $L_2$ cost is chosen in this paper. While the greedy minimization makes the algorithm sensitive to initialisation, the ability to converge from any initial guess to a local optimum allows the algorithm to be integrated into other existing algorithms. Three variants of the algorithm are tested over a large number of synthetic datasets, one being a standalone LM implementation, and two others that combine with existing algorithms. One of the latter two -- LM-enhanced-Bottom-Up segmentation -- is found to have the best accuracy and the lowest computational complexity among all algorithms. This variant of LM can provide $k$-segmentations over data sets with up to a million image frames within several seconds.

==> figures/algo_avg_met_Nk_xss_base_SN.tex <==
\begin{tabular}{lrrrr}
\toprule
    Algorithm &  Rel. runtime &  Rel. cost &  Covering &  Rand Index \\
\midrule
    SNBC\_sf50 &         0.349 &      1.182 &     0.979 &       0.995 \\
    SNBC\_sf10 &         0.170 &      1.138 &     0.976 &       0.993 \\
 SNBC\_sf10-LM &         0.177 &      1.066 &     0.983 &       0.997 \\
        BotUp &         0.086 &      2.132 &     0.969 &       0.990 \\
     LM-BotUp &         0.045 &      1.829 &     0.965 &       0.990 \\
           SN &         1.000 &      1.000 &     0.982 &       0.997 \\
   LM\_20inits &         0.360 &      1.501 &     0.929 &       0.981 \\
         PELT &         6.365 &      1.920 &     0.923 &       0.969 \\
           BS &         0.279 &      1.724 &     0.894 &       0.967 \\
\bottomrule
\end{tabular}

